Majorization Minimization Methods for Distributed Pose Graph Optimization

We consider the problem of distributed pose graph optimization (PGO) that has important applications in multi-robot simultaneous localization and mapping (SLAM). We propose the majorization minimization (MM) method for distributed PGO ($\mathsf{MM-PGO}$) that applies to a broad class of robust loss kernels. The $\mathsf{MM-PGO}$ method is guaranteed to converge to first-order critical points under mild conditions. Furthermore, noting that the $\mathsf{MM-PGO}$ method is reminiscent of proximal methods, we leverage Nesterov's method and adopt adaptive restarts to accelerate convergence. The resulting accelerated MM methods for distributed PGO -- both with a master node in the network ($\mathsf{AMM-PGO}^*$) and without ($\mathsf{AMM-PGO}^{\#}$) -- have faster convergence in contrast to the $\mathsf{AMM-PGO}$ method without sacrificing theoretical guarantees. In particular, the $\mathsf{AMM-PGO}^{\#}$ method, which needs no master node and is fully decentralized, features a novel adaptive restart scheme and has a rate of convergence comparable to that of the $\mathsf{AMM-PGO}^*$ method using a master node to aggregate information from all the other nodes. The efficacy of this work is validated through extensive applications to 2D and 3D SLAM benchmark datasets and comprehensive comparisons against existing state-of-the-art methods, indicating that our MM methods converge faster and result in better solutions to distributed PGO.

==> acknowledgement.tex <==
This material is partially based upon work supported by the National Science Foundation under award DCSD-1662233. Any opinions, findings, and conclusions or recommendations expressed in this material are those of the authors and do not necessarily reflect the views of the National Science Foundation. We thank Yulun Tian for kindly sharing the code of Riemannian block coordinate descent method ($\rbcd$) for distributed PGO \cite{tian2019distributed}.

==> algorithm_amm_phi.tex <==
\begin{algorithm}[t]
	\caption{Update $F^{\aab(\skp)}$ for the $\ammd$ Method}
	\label{algorithm::amm_phi}
	\begin{algorithmic}[1]
	\State $\!F^{\ab(\skp)}\gets F^{\ab}(\Xkp)$ using \cref{eq::Fab3}\label{line::alg7::Fabkp}
	\vspace{0.1em}
	\State $\!E^{\ab(\skp)}\gets E^{\ab}(\Xkp|\Xk)$ using \cref{eq::Eab3}\label{line::alg7::Eabkp}
	\vspace{0.1em}
	\State $\!E^{\aab(\skp)} \!\gets\!  E^{\aab}(\Xakp|\Xk) + F^{\aab(\sk)}$ using \cref{eq::Eaab}\label{line::alg7::Eaabkp}
	\vspace{-0.75em}
	\State $F^{\aab(\skp)}\gets E^{\aab(\skp)} + \frac{1}{2}\big(F^{\ab(\skp)}-E^{\ab(\skp)}\big)$\label{line::alg7::Faabkp}
	\end{algorithmic}
\end{algorithm}

==> biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/fan.png}}]{Taosha Fan}
received his B.E. degree in automotive engineering from Tongji University, Shanghai, China, in 2013, and M.S. degrees in mechanical engineering and mathematics from Johns Hopkins University, Baltimore, MD, USA, in 2015. He is currently a Ph.D. candidate in mechanical engineering at Northwestern University, Evanston, IL, USA. His research interests lie at the intersection of robotic control, simulation and estimation.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/murphey.png}}]{Todd Murphey}
received his B.S. degree in mathematics from the University of Arizona and the Ph.D. degree in Control and Dynamical Systems from the California Institute of Technology.
He is a Professor of Mechanical Engineering at Northwestern University. His laboratory is part of the Neuroscience and Robotics Laboratory, and his research interests include robotics, control, computational methods for biomechanical systems, and computational neuroscience.
Honors include the National Science Foundation CAREER award in 2006, membership in the 2014-2015 DARPA/IDA Defense Science Study Group, and Northwestern’s Professorship of Teaching
Excellence. He was a Senior Editor of the IEEE Transactions on Robotics.
\end{IEEEbiography}

==> fig_cube_results_robust.tex <==
\begin{figure*}[t]
	\centering
	\begin{tabular}{cccc}
		\hspace{-0.5em}\subfloat[][$\ammd$ vs. $\mm$]{\includegraphics[trim =0mm 0mm 0mm 0mm,width=0.24\textwidth]{figures/cube_tests/rel_huber_g.png}} &
		\hspace{-0.6em}\subfloat[][5 robots]{\includegraphics[trim =0mm 0mm 0mm 0mm,width=0.24\textwidth]{figures/cube_tests/rel_huber_g_5.png}} &
		\hspace{-0.6em}\subfloat[][10 robots]{\includegraphics[trim =0mm 0mm 0mm 0mm,width=0.24\textwidth]{figures/cube_tests/rel_huber_g_10.png}}&
		\hspace{-0.6em}\subfloat[][50 robots]{\includegraphics[trim =0mm 0mm 0mm 0mm,width=0.24\textwidth]{figures/cube_tests/rel_huber_g_50.png}}
	\end{tabular}
	\caption{The Riemannian gradient norms of the $\mm$, $\ammc$, $\ammd$ and $\amm$ \cite{fan2020mm} methods for distributed PGO with the \textbf{Huber loss kernel} on $5$, $10$ and $50$ robots. The results are averaged over $20$  Monte Carlo runs.}\label{fig::cube_g_huber} 
	\vspace{-0.5em}

	\begin{tabular}{cccc}
		\hspace{-0.5em}\subfloat[][$\ammd$ vs. $\mm$]{\includegraphics[trim =0mm 0mm 0mm 0mm,width=0.24\textwidth]{figures/cube_tests/rel_welsch_g.png}} &
		\hspace{-0.6em}\subfloat[][5 robots]{\includegraphics[trim =0mm 0mm 0mm 0mm,width=0.24\textwidth]{figures/cube_tests/rel_welsch_g_5.png}} &
		\hspace{-0.6em}\subfloat[][10 robots]{\includegraphics[trim =0mm 0mm 0mm 0mm,width=0.24\textwidth]{figures/cube_tests/rel_welsch_g_10.png}}&
		\hspace{-0.6em}\subfloat[][50 robots]{\includegraphics[trim =0mm 0mm 0mm 0mm,width=0.24\textwidth]{figures/cube_tests/rel_welsch_g_50.png}}
	\end{tabular}
	\caption{The Riemannian gradient norms of the $\mm$, $\ammc$, $\ammd$ and $\amm$ \cite{fan2020mm} methods for distributed PGO with the \textbf{Welsch loss kernel} on $5$, $10$ and $50$ robots. The results are averaged over $20$  Monte Carlo runs.}\label{fig::cube_g_gm}
	\vspace{-0.75em}
\end{figure*}


==> fig_cube_results_trivial.tex <==
\begin{figure*}[t]
	\centering
	\begin{tabular}{cccc}
		\hspace{-0.5em}\subfloat[][$\ammd$ vs. $\mm$ ]{\includegraphics[trim =0mm 0mm 0mm 0mm,width=0.24\textwidth]{figures/cube_tests/rel_none_f.png}} &
		\hspace{-0.6em}\subfloat[][5 robots]{\includegraphics[trim =0mm 0mm 0mm 0mm,width=0.24\textwidth]{figures/cube_tests/rel_none_f_5.png}} &
		\hspace{-0.6em}\subfloat[][10 robots]{\includegraphics[trim =0mm 0mm 0mm 0mm,width=0.24\textwidth]{figures/cube_tests/rel_none_f_10.png}}&
		\hspace{-0.6em}\subfloat[][50 robots]{\includegraphics[trim =0mm 0mm 0mm 0mm,width=0.24\textwidth]{figures/cube_tests/rel_none_f_50.png}}
	\end{tabular}
	\caption{The relative suboptimality gaps of the $\mm$, $\ammc$, $\ammd$ and $\amm$ \cite{fan2020mm} methods for distributed PGO with the \textbf{trivial loss kernel} on $5$, $10$ and $50$ robots. The results are averaged over $20$  Monte Carlo runs.}\label{fig::cube_f} 
	\vspace{-1em}
\end{figure*}
